Towards Assessing and Characterizing the Semantic Robustness of Face Recognition

Deep Neural Networks (DNNs) lack robustness against imperceptible perturbations to their input. Face Recognition Models (FRMs) based on DNNs inherit this vulnerability. We propose a methodology for assessing and characterizing the robustness of FRMs against semantic perturbations to their input. Our methodology causes FRMs to malfunction by designing adversarial attacks that search for identity-preserving modifications to faces. In particular, given a face, our attacks find identity-preserving variants of the face such that an FRM fails to recognize the images belonging to the same identity. We model these identity-preserving semantic modifications via direction- and magnitude-constrained perturbations in the latent space of StyleGAN. We further propose to characterize the semantic robustness of an FRM by statistically describing the perturbations that induce the FRM to malfunction. Finally, we combine our methodology with a certification technique, thus providing (i) theoretical guarantees on the performance of an FRM, and (ii) a formal description of how an FRM may model the notion of face identity.

==> Figures/anisotropic-certification.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{Images/equivrad-anisotropic-certification-compare.png}
    \vspace{-0.6cm}
    \caption{\textbf{Certifying Face Recognition Models via Anisotropic Randomized Smoothing.}
    We explore the anisotropic setting in our certification methodology, allowing us to introduce \textit{a priori} knowledge about the subspace of certification.
    We apply anisotropic Randomized Smoothing on each model, and report the corresponding certification curves (first three plots) and the envelope curves in the right-most plot.}
    \label{fig:anisotropic-certification-comparison}
\end{figure*}

==> Figures/fab-attacks.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Images/FAB-attacks-compare.png}
    \vspace{-0.6cm}
    \caption{\textbf{Accuracy \textit{vs.} perturbation budget under FAB attacks.}
    We find semantic adversarial examples for Face Recognition Models with FAB, and show how accuracy steadily drops as the perturbation budget increases.
    }
    \label{fig:fab-comparison}
\end{figure}

==> Figures/isotropic-certification.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{Images/certification-compare.png}
    \vspace{-0.6cm}
    \caption{\textbf{Certifying Face Recognition Models (FRMs) via Randomized Smoothing (RS).} 
    We apply RS on each FRM model and plot the corresponding certification curves in the first three plots.
    Each plot shows the curves obtained by smoothing with individual $\sigma$s and the associated envelope curve.
    The right-most plot compares the FRMs by contrasting their envelope curves.
    }
    \label{fig:certification-comparison}
\end{figure*}

==> Sections/design_choices.tex <==
\section{Design Choices}
\paragraph{Defining $V$.}
Matrix $V$ is the set of directions associated with semantic attributes in faces.
To derive $V$, we draw upon InterFaceGAN~\cite{shen2020interfacegan,shen2020interpreting}, a recent method that discovers interpretable directions in StyleGAN's latent space.
These directions allow control of a face's semantic attributes.
Thus, we build matrix $V$ from the set of $N = 5$ direction vectors provided by InterFaceGAN, which correspond to
% that this method provides for the 
attributes ``Pose'', ``Age'', ``Gender'', ``Smile'' and ``Eyeglasses''.

\paragraph{Defining $M$.}
Matrix $M$ characterizes the ellipsoid of valid perturbations $\pmb{\delta}$ by controlling their norm via $\|\pmb{\delta}\|_{M, 2} \leq 1$.
Each entry of $\pmb{\delta} \in \mathbb{R}^N$ is associated with one direction from $\{\mathbf{v}_i\}_{i=1}^N$, which, in turn, corresponds to a semantic attribute.
Defining $M$ is thus linked with the \textit{maximum} amount of perturbation allowed along each individual direction $\mathbf{v}_i$.
Let the scalar $\epsilon_i$ state the maximum extent to which latent codes can be perturbed along $\mathbf{v}_i$, then, in terms of $\pmb{\delta}$, we have the condition $|\pmb{\delta}_i| \leq \epsilon_i$.
Unfortunately, combining this condition with the fact that $M$ must characterize an ellipsoid still leaves $M$'s definition ill-posed.
To solve this ambiguity, we additionally require $M$ to enclose the minimum possible volume.
Under this formulation, we find that $M$ must be a diagonal matrix whose elements are the reciprocal of the squares of the $\epsilon$, that is $M = \text{diag}(\epsilon_1^{-2},\:\dots, \:\epsilon_N^{-2})$.
We leave the details of this derivation and its benefits in downstream computational costs to the \textbf{Supplementary Materials}.

==> Sections/experiments.tex <==
\section{Experiments}
In this section, we assess and characterize the semantic robustness of off-the-shelf Face Recognition Models with our methodology.
% We start in Section~\ref{sec:visualize} by visualizing identity-preserving variants of faces (as defined via the set $\mathcal{V}(I)$ from Section~\ref{sec:semantic_perturbs}).
We first study robustness under constrained-perturbation attack, \ie PGD.
Then, we study robustness under minimum-perturbation attack, \ie FAB.
Finally, we run both isotropic and anisotropic certifications on the FRMs.

\subsection{Experimental details}
\paragraph{Models.} 
We target three renowned off-the-shelf FRMs: \textit{(i)} ArcFace~\cite{deng2019arcface}, \textit{(ii)} a FaceNet~\cite{schroff2015facenet} model trained on CASIA-Webface~\cite{yi2014learning}, which we refer to as ``FaceNet$^C$'', and \textit{(iii)} a FaceNet model trained on VGGFace2~\cite{cao2018vggface2}, which we refer to as ``FaceNet$^V$''\footnote{All models were retrieved from the well-known public implementations \texttt{InsightFace} and \texttt{facenet-pytorch}}.

\paragraph{Attributes' budget.} 
In Table~\ref{tab:attribute-budgets} we report the budgets assigned to each attribute, that is, the scalars $\epsilon_i$ that state the maximum extent to which a latent code can be perturbed in the direction corresponding to each attribute.
These values were established by a qualitative exploration of StyleGAN's output.
In particular, we aimed at establishing these values such that, after a perturbation of at most these magnitudes, StyleGAN's could still generate high-quality images of faces that, arguably, belong to the original identity.
\input{Tables/attributes_budget}

\paragraph{Attacks.}
Unless stated otherwise, we always experiment with a \texttt{100k}-identity dataset (of comparable size to FFHQ~\cite{karras2019style}), from which we extract \texttt{5k} identities to attack.
\underline{\textit{PGD attack.}}
We use PGD with 10 iterations and 10 restarts.
We provide ablations of these two hyper-parameters in the \textbf{Supplementary Materials}.
\underline{\textit{FAB attack.}}
The FAB attack has un-targeted and targeted versions.
The computational cost of FAB's un-targeted version scales with the number of output classes.
Since FRMs cast identities as individual classes, the cost's dependence on the number of classes renders FAB's un-targeted version intractable for our purposes.
Thus, in practice, we use the \textit{targeted} version of FAB, or ``FAB-t''.
However, to avoid cluttering throughout the experiments, we will refer to this attack simply as FAB.
For FAB we use 10 iterations, 10 restarts and 10 target classes (\ie the number of classes for which the targeted attack is run).
We provide ablations of these three hyper-parameters in the \textbf{Supplementary Materials}.

\paragraph{Certification.}
Randomized smoothing (RS)-based certification is based on a Monte Carlo method and a statistical test on the estimated probability of the predicted class.
We use $n = 10,000$ samples for the Monte Carlo estimate, and a confidence of $\alpha = 10^{-3}$ for the statistical test.
Due to RS' large computational requirements, we follow common practice~\cite{cohen2019certified} and certify 500 instances, \ie 500 identities.

% \subsection{Identity-preserving Variants of Images}\label{sec:visualize}
% In Figure~\textcolor{red}{X} we select four identities and visualize three samples from their corresponding identity-preserving neighborhoods. 
% We argue that the samples drawn from each neighborhood would be judged by human observers as belonging to the same person.


\subsection{Attacks with PGD}\label{sec:pgd_attacks}
Attacking each FRM with PGD reveals the model's semantic robust accuracy.
We find that these robust accuracies are: 84.9 for ArcFace, 76.9 for FaceNet$^C$, and 71.0 for FaceNet$^V$. 
That is, PGD attacks suggest that ArcFace is more robust than FaceNet$^C$, which is, in turn, more robust than FaceNet$^V$.

\input{Figures/pgd_examples}

We show a sample of the adversarial examples that fooled an FRM in Figure~\ref{fig:pgd_results}.
We qualitatively inspect the examples found by PGD, and find that eyeglasses are a prevalent feature in...

\input{Tables/attr_ranking_pgd}

\paragraph{Characterizing semantic robustness.}
We can characterize an FRM's semantic robustness by applying the procedure described in Section~\ref{sec:interpreting} on the semantic adversarial examples that PGD found for that FRM.
Under the assumption that the induced perturbations indeed result in identity-preserving modifications, an adversarial example for person \underline{A} can be interpreted as \textit{``a variant of \underline{A}'s face that the FRM fails at recognizing as \underline{A}''}.
Since these examples were found via a constrained-perturbation attack, the relative energy spent by the attack on modifying each attribute relates to the FRM's sensitivity to such attribute.
Thus, we argue that the relative energy spent on modifying an attribute can be interpreted as related to \textit{``the FRM's disproportionate sensitivity to modifications on such attribute''}.

We run the aforementioned procedure and report the ranking we obtain in Table~\ref{tab:deltas_pgd}.
From this ranking, we mark three main observations that hold for all FRMs: \textit{(i)} the ``Eyeglasses'' attribute leads the ranking in 1$^{\text{st}}$ position, \textit{(ii)} the ``Pose'' and ``Age'' attributes take either the 2$^{\text{nd}}$ or 3$^{\text{rd}}$ position, and \textit{(iii)} the ``Smile'' and ``Gender'' attributes take the last two positions (4$^{\text{th}}$ and 5$^{\text{th}}$).

We interpret these observations as follows.
The presence/absence of eyeglasses is a strong cue on which FRMs rely on (somewhat disproportionately) for recognizing individuals.
This phenomenon is inconvenient and suggests avenues for improving FRMs.
However, we also relate the FRMs' sensitivity to eyeglasses with the difficulty humans experience when recognizing a person who recently started/stopped wearing eyeglasses.
Since humans are a strong baseline for FRMs, we argue that requesting FRMs to not rely on such cue may prove unreasonable.
Most likely, thus, the most practical solutions to this problem are to either \textit{(i)} store images of the person's face with and without eyeglasses in the database, or \textit{(ii)} always ask the person to remove eyeglasses before using an FRM.
The inconvenience introduced by either solution calls for more sophisticated ways of handling the FRMs' sensitivity to eyeglasses.

The FRMs' large sensitivity to the next two attributes (pose and age) is interesting.
For age, analogous to our previous comment on eyeglasses, humans also have trouble recognizing faces when the person's age strongly varies between the face they were originally presented with and the new face (\eg, when seeing someone's old picture or when seeing them after a large amount of time).
That is, age can introduce salient changes to faces that hinder the human capacity to recognize them.
We further found, as judged by our qualitative inspection, that while GANs provide remarkably plausible examples of how a person might look younger/older, the quality of these examples degrades significantly when the person's apparent age is close to that of a child.
This phenomenon stems from the fact that facial cues vary drastically during the transition from child to adult.
Regarding pose, we find that indeed some FRMs can be fooled by almost exclusively modifying the face's pose.
However, we also observe that the FRMs' failure in some of these cases can be mostly attributed to a malfunction of the GAN, which introduces well-known artifacts when queried with generating ``extreme'' poses.

Finally, the smile and gender attributes fall last in the ranking.
Thus, compared to other attributes, \textit{neither} smile nor gender are attributes to which FRMs are disproportionately sensitive.
This result can be understood as a satisfying result.
Under the constrained budget we allow for the attack, modifying either smile or gender is largely ineffective: altering either attribute \textit{such that} the FRM is fooled would require a magnitude that is simply not attainable given the constraint.
Changing a person's smile such that an FRM changes its prediction is impractical.
Similarly, changing a person's gender under a constrained budget is virtually unfeasible.

A brute-force approach to characterizing semantic robustness against modifications of individual attributes can also be considered.
This approach would consist of constraining PGD's search to individual directions, which is accomplished by defining both matrices $V$ and $M$ based solely on the attribute of interest.
We run this experiment and obtain results consistent with the ones reported here.
We leave experimental details and results for the \textbf{Supplementary Materials}.

\input{Figures/pgd_exps}

\paragraph{Robustness \textit{vs.} dataset's size.}
As the dataset varies in size, an FRM's chances of confusing individuals change.
A larger (or smaller) pool of individuals implies larger (or smaller) probabilities for the dataset to contain individuals with similar facial features.
Hence, this factor affects our assessment of an FRM's robustness.

We thus control for this factor by modifying the number of identities in the dataset and conducting PGD attacks on the same \texttt{5k} samples as before.
We vary the dataset's size from the original \texttt{100k} identities to as little as \texttt{5k} and as much as \texttt{1M}.
Figure~\ref{fig:pgd_vs_n_ids} reports the robust accuracies for each of the dataset sizes we considered.
As expected, the robust accuracies of all FRMs start at high values when the dataset is small and then drop rapidly as the number of identities increases (notice the x-axis' \textit{log} scale).
In particular, performances drop from around 85 when there are \texttt{5k} identities to around 70 when there are \texttt{1M} identities.
Namely, performances change as follows: ArcFace: $93.0\to77.9$, FaceNet$^C$: $85.5\to70.9$, and FaceNet$^V$: $81.4\to64.7$.

Our experiments show that an FRM's semantic robustness depends largely on the number of identities it is required to recognize.
In turn, this number of identities is conditioned on the particular setting in which the FRM is deployed.
Hence, depending on the deployment setting, the concern regarding semantic robustness may vary from negligible to worrisome.


\paragraph{Sample representativeness.}
For computational feasibility, our testbed for all attacks consisted of a sample of \texttt{5k} out of the \texttt{100k} identities.
Here we test whether this set of identities is a representative sample of the population.
We thus fix the \texttt{100k} identities in the dataset, and vary the amount of samples we attack from \texttt{1k} to \texttt{20k}.
We report results for this experiment in Figure~\ref{fig:pgd_on_n_ids}.
Our experiments show that there is virtually no variation in the semantic robustness of any FRM.
These results suggest that our design choice of experimenting on \texttt{5k} samples provides a reasonable sample of the population.
Hence, this results implies that semantic adversarial robustness can be assessed with a ``sensible'' amount of samples.


\paragraph{Perturbation budget.}
In the previous experiments, we search for adversarial examples within the volume enclosed by an ellipsoid of a fixed volume.
The volume of this ellipsoid is directly related to the budget we allow for the perturbation: the larger the volume, the larger the perturbation can be, and hence the stronger the attack.
Here we test how FRMs behave under budgets different from the one we initially considered.
In particular, given the original constraint of $\| \pmb{\delta}\|_{M, 2} \leq \epsilon = 1$, we vary the budget, \ie $\epsilon$, from as little as $\nicefrac{1}{4}$ to as much as $8$ and record each FRM's robustness.
This interval varies from the most conservative (small perturbation) to the least realistic (large perturbation) scenarios.
We report results for this experiment on Figure~\ref{fig:pgd_pert_budget}.
These results show that robustness against semantic perturbations drops rapidly when the perturbation budget increases: for all FRMs, robustness drops from around 95 for a small budget of $\epsilon = \nicefrac{1}{4}$, to around 5 for a large budget of $\epsilon = 8$.
Specifically, performances change as follows: ArcFace: $98.3\to4.1$, FaceNet$^C$: $95.4\to12.6$, and FaceNet$^V$: $93.3\to7.3$.

For small budgets of $\epsilon < 1$, we observe that the FRM ranking we found earlier is preserved: ArcFace $>$ FaceNet$^C$ $>$ FaceNet$^V$.
However, this ranking changes for large budgets of $\epsilon > 1$, as ArcFace goes from leading the ranking to occupying the last position.
While this change in ranking draws attention, we argue that the impact on practical applications is rather negligible, as the modifications allowed by a large budget, while still being mostly semantic, no longer seem to preserve identity.


\subsection{FAB attack}\label{sec:fab_attacks}
We also assess each FRM's semantic robust accuracy through attacks with FAB.
The FAB attack aims at minimum perturbation, in contrast to PGD's constrained perturbation.
Thus, while FAB does search over the subspace of semantic attributes, there is no guarantee that the adversarial examples found by FAB lie in the identity-preserving neighborhood we introduced in Section~\ref{sec:method}.
In particular, we remark that FAB can successfully find adversarial examples for \textit{all} the instances it is tasked with attacking; however, the found examples may no longer be judged by a human observer as belonging to the same identity.
We consider this characteristic of the adversarial examples found by FAB when interpreting the results in this section.

\input{Figures/fab-attacks}

We run FAB on each of the FRMs we consider, and find semantic adversarial examples for all the \texttt{5k} identities we attack.
The latent code $\mathbf{w}^\prime = \mathbf{w} + V^\top\pmb{\delta}$ of each adversarial example we find has an associated perturbation budget of $\| \pmb{\delta}\|_{M, 2}$.
Thus, following common practice in adversarial robustness~\cite{dong2020benchmarking}, we evaluate a model's robustness by plotting its accuracy \textit{vs.} perturbation budget curve.
We report such curves for all FRMs in Figure~\ref{fig:fab-comparison}.
Adversarial robustness is associated with how the curve of each FRM shows steady accuracies as the perturbation budget increases.
Thus, according to FAB's assessment of semantic adversarial robustness, ArcFace is more robust than FaceNet$^C$, which, in turn, is more robust than FaceNet$^V$.
That is, the ranking we found by FAB agrees with the ranking we found via PGD.
This experiment suggests that our assessment of semantic adversarial robustness is self consistent.

\paragraph{Characterizing semantic robustness.}
We characterize semantic robustness by analyzing the adversarial examples found by FAB and obtaining a ranking of attributes.
This procedure shares spirit with the one for PGD-based adversarial examples (from Section~\ref{sec:pgd_attacks}).
However, this ranking \textit{cannot} be interpreted in the same way we interpreted the one we obtained when using PGD.
FAB is tasked with finding adversarial examples for \textit{every} identity while minimizing the perturbation induced in the identity.
Consequently, the adversarial examples found by FAB need not belong to the identity of the person the attack was targeting.
That is, an adversarial example for person \underline{A} can be interpreted as \textit{``a face of a person that shares facial attributes with \underline{A} (to some extent) yet is classified as different from \underline{A} by the FRM''}.
Thus, we argue that the relative energy spent on modifying an attribute can be interpreted as related to \textit{``the FRM's reliance on such attribute''}.

\input{Tables/attr_ranking_fab}

We report the attribute ranking we generate in Table~\ref{tab:deltas_fab}.
From this ranking, we mark two main observations that hold for all FRMs: \textit{(i)} the attributes ``Gender'', ``Pose'' and ``Eyeglasses'' always come up in the 1$^{\text{st}}$ to 3$^{\text{rd}}$ positions, and \textit{(ii)} the 4$^{\text{th}}$ and 5$^{\text{th}}$ positions are occupied, respectively, by ``Age'' and ``Smile''.

We interpret the first observation as follows.
First, the fact that ``Gender'' occupies early positions in the ranking is reasonable, as human's most likely also rely heavily on the attributes they customarily associate with gender.
That is, it follows intuitive sense that an FRM would also rely on this informative cue to recognize human faces.
Similarly, seeing ``Eyeglasses'' prompt in the first positions also agrees with our previous observations from Section~\ref{sec:pgd_attacks}, in which we notice FRMs' striking difficulty for recognizing faces when glasses are added/removed.
While the reliance on either ``Gender'' or ``Eyeglasses'' points to a direction for improving FRMs, we argue it is difficult to question that FRMs learn dependence on these cues, as humans also do.
In contrast, the early position that the ``Pose'' occupies is surprising.
We are unable to give a reasonable explanation to why FRMs would rely on the signal conveyed by ``Pose''.
Thus, we attribute this case of failure of our methodology to the artifacts that StyleGAN introduces in faces when handling extreme poses.

We interpret the second observation as follows.
The fact that ``Smile'' ranks last is satisfactory.
Indeed, FRMs should not be expected to rely much on the ``degree'' of smile to recognize a human face.
However, the fact that ``Age'' ranks relatively low (4$^{\text{th}}$ on a ranking of five attributes), requires careful interpretation.
In particular, we make two remarks.
First, a ranking is, inherently, a \textit{relative} comparison of importance.
That is to say, ``Age'' ranking 4$^{\text{th}}$ does not mean that FRMs \textit{do not} rely on a person's age to recognize them, but rather that they rely less on the person's age than on the other attributes we considered.
Additionally, qualitative inspection of the age-manipulated faces suggests that modifying age is rather unstable.
We argue that modeling age with a single direction vector (independent of the original face) can result in unpredictable outcomes; for instance, varying a child's age \textit{rapidly} changes several attributes, while varying an adult's face by the same amount changes fewer.
Ultimately, we think that some of the cases of failure we observe can be, for the most part, attributed to the instability of GAN's output \textit{and} the problems associated with adequately modeling disentangled manipulation of attributes.

Analogous to our experiments with PGD, one can also consider a brute-force approach for characterizing semantic robustness against modifications of individual attributes.
We run this experiment and obtain results consistent with the ones reported here.
We report detailed experimental settings and results in the \textbf{Supplementary Materials}.

Ablate each direction: what if FAB is given access only to one direction?
How do the adversaries look like, and what is the magnitude of the found perturbation.

\subsection{Certification}
\paragraph{Isotropic certification.} Following the methodology we introduced in Section~\ref{sec:certification}, we certify all FRMs with covariance $\Sigma = \sigma^2\pmb I$, and set $\sigma \in \{0.1, 0.25, 0.5, 0.75, 1\}$.
For each identity, \ie latent code, and $\sigma$ value, Randomized Smoothing (RS) returns a quantity known as the certification radius.
This quantity states that the classifier's prediction on the corresponding latent code will remain constant as long as the perturbation applied to the latent code is below this quantity.
By aggregating the certification radii for all identities we can construct certification curves~\cite{cohen2019certified}.
Each point $(x,y)$ in this curve asserts the fraction $y$ of the dataset for which the prediction of the smooth classifier $g$ from Eq.~\ref{def:smooth-classifier} is certifiably robust within an $\ell_2$ ball of radius $x$.

Figure~\ref{fig:certification-comparison} reports the certification curves for each FRM, together with the curves' associated envelope, \ie the largest certificate that can be granted to each identity across the $\sigma$ values considered.
Our results for certification of each FRM are analogous to those for certification of classifiers operating on natural images~\cite{cohen2019certified}. 
Specifically, for a given FRM we note: \textit{(i)} all curves are monotonically decreasing, \textit{(ii)} the left-most point in each curve is higher as $\sigma$ is smaller, and \textit{(iii)} the height of each curve's left-most point is inversely related to how fast the curve drops as the radius increases.
Furthermore, when comparing across FRMs via the right-most plot in Figure~\ref{fig:certification-comparison}, we again find the ranking obtained via PGD and FAB attacks: ArcFace $>$ FaceNet$^C$ $>$ FaceNet$^V$.
This finding again suggests that our assessment of semantic robustness is self consistent.

The region of certification we find in these experiments may have provide insights into the FRM being certified.
In particular, we argue that the certification region (for a given identity and FRM) can be interpreted as a subset of what the FRM understands the person to \textit{be}. 
In other words, with respect to the FRM, everything inside a person's certification region corresponds to the person herself.
Thus, in a sense, this region is related to the FRM's notion of ``identity''.

\input{Figures/isotropic-certification}


\paragraph{Anisotropic certification.}
The original RS work studied the case of isotropic certification, \ie the covariance took the form $\Sigma = \sigma^2\pmb I$.
However, assuming isotropy in the subspace of semantic attributes we consider in this work (modeled by matrix $V$) is unsubstantiated.
% and, most likely, unreasonable given the nature of the attributes and the approach.
Thus, we explore anisotropic certification by drawing upon recent work~\cite{ancer} that extended RS to the anisotropic setting.
For exploiting this avenue, we are required to provide a sensible candidate matrix $\Sigma$ that encodes \textit{a priori} knowledge we have on the subspace of semantic attributes.
Thus, we set $\Sigma = M^{-1}$, where $M$ is the matrix encoding the magnitude constraints in our approach.
The rationale behind this decision is that the Mahalanobis distance to the distribution $\mathcal{N}(0,M^{-1})$ will draw precisely the shape of the ellipsoid characterized by $M$.

\input{Figures/anisotropic-certification}

For the experiments, we consider $\Sigma = \sigma M^{-1}$ and set $\sigma \in \{0.25, 0.5, 0.75, 1, 2, 2.5\}$.
Certification of anisotropic regions renders the notion of certified radius meaningless, since such regions cannot be characterized by a single radius.
Consequently, we compute an ``Equivalent-volume radius'', \ie the radius of a ball whose volume is that of the certified region, and then report the certification curves for each FRM in Figure~\ref{fig:anisotropic-certification-comparison}.
Our observations from this experiment are consistent with those from the isotropic case.
Worthy of mention, in the right-most plot of Figure~\ref{fig:anisotropic-certification-comparison} we again find the ranking of FRMs we obtained via all previous experiments: ArcFace $>$ FaceNet$^C$ $>$ FaceNet$^V$.

This experiment demonstrates that anisotropic certification is a feasible and interesting alternative for certification that allows inductive biases to be encoded into the certification process.
Our experiments show that the selection of covariance matrix was, to some extent, reasonable, as demonstrated by the magnitudes of Area-Under-the-Curve metrics reported in Figure~\ref{fig:anisotropic-certification-comparison}.
However, the fact that none of these values exceed the corresponding values from the isotropic setting means that a better choice of covariance matrix could be made.


\begin{comment}
Compare isotropic \textit{vs.} anisotropic certificates in Figure~\ref{fig:anisotropic-isotropic-comparison}.
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{Images/anisotropic-isotropic-comparison.png}
    \caption{\textbf{Comparison between isotropic and anisotropic certificates.} As the certification radius increases...}
    \label{fig:anisotropic-isotropic-comparison}
\end{figure}
\end{comment}


==> Sections/methodology.tex <==
% \section{Methodology}\label{sec:methodology}
% Most adversarial attacks aim at fooling a recognition model by imperceptibly modifying its input through an additive perturbation in pixel space.
% These attacks find such a perturbation by searching for incorrectly-classified images on a set of imperceptible perturbations.
% This set of imperceptible perturbations in pixel space is usually defined as an $\ell_p$ ball with a small radius $\epsilon$, where the aim of this constraint is to ensure the semantics of the image are preserved.
% Thus, these attacks find perturbations that leave both the image \textit{and} its semantics mostly unchanged.

% In contrast, our work aims at conducting semantically-viable adversarial attacks: finding a semantically-viable perturbation that (most likely) visibly perturbs an input image while leaving its semantics unchanged.
% To achieve this purpose, we diverge from perturbing the pixel space, and rather turn to perturbing the image-generating process.
% In particular, we model the image-generating process with a GAN, and cast the set of semantically-viable perturbations as a constrained region of a linear subspace in the GAN's latent space.
% We induce semantic properties on this region via \textit{(i)} the selection of constraints imposed on this region, and \textit{(ii)} the selection of the subspace.
% By defining such a region, we can define a semantically-viable adversarial attack as searching for incorrectly-classified images on our set of semantically-viable perturbations.

% Next, we present (1) the formal definition of semantically-viable perturbations, (2) their associated adversarial attacks, (3) our theoretical results for certifying recognition systems against semantic perturbations, and (4) practical considerations for implementing our approach in practice.


% \subsection{Semantically-viable Perturbations}\label{sec:semantic_perturbs}
% A generative model $G: \mathcal{Z} \to \mathcal{I}$ can produce images by mapping from a latent space to the image space. 
% We consider a latent code $\mathbf{z} \in \mathcal{Z} \subseteq \mathbb{R}^d$, which produces image $I = G(\mathbf{z})$.
% A perturbed variant of image $I$ can be generated with additive perturbations on $\mathbf{z}$, as $I^p = G(\mathbf{z} + \pmb{\eta})$, where $\pmb{\eta} \in \mathbb{R}^d$ is a noise vector.
% However, we are not interested in \textit{any} kind of noise, but rather noise that produces semantically-viable perturbations.
% Thus, we model semantically-viable perturbations on image $I$ as direction- and magnitude-constrained additive perturbations on $\mathbf{z}$, \ie by imposing constraints on $\pmb{\eta}$.
% Next, we describe how we model each of these constraints.

% \textbf{Direction constraints.} 
% We are interested in perturbations $\pmb{\eta}$ that follow a set of $N$ directions $\{\mathbf{v}_i\}_{i=1}^N$, where $\mathbf{v}_i \in \mathbb{R}^d$.
% If we vertically stack these direction vectors into matrix $V \in \mathbb{R}^{N \times d}$, we note that the direction constraint amounts to enforcing $\pmb{\eta}$ to lie in the subspace spanned by the rows of $V$.
% This constraint is easily enforced by setting $\pmb{\eta} = V^\top\pmb{\delta}$, where $\pmb{\delta} \in \mathbb{R}^N$.

% \textbf{Magnitude constraints.} 
% Given our approach to enforcing the direction constraints, we do not directly constrain the magnitude of $\pmb{\eta}$, but rather the magnitude of $\pmb{\delta}$.
% Most works in adversarial robustness constrain the perturbation in the sense of the perturbation's $\ell_p$ norm.
% However, we note that this scheme inherently assumes an over-simplistic interaction of components by inducing isotropy in the perturbation's norm.
% This effect can be undesirable for our purposes: the scale in which semantic attributes are changed may not be comparable across attributes. 
% Thus, to allow for anisotropy, we abstain from formulating the magnitude constrain in the sense of the traditional $\ell_p$ norms.
% Rather, we introduce a symmetric and Positive-Definite (PD) matrix $\Sigma \in \mathbb{R}^{N \times N}$, and consider the product between $N$-dimensional vectors $\mathbf{u}$ and $\mathbf{v}$ as the bilinear form $M_\Sigma(\mathbf{u},\mathbf{v}) = \mathbf{u}^\top\Sigma\:\mathbf{v}$.
% Given this function, we model the constraint on $\pmb{\delta}$'s magnitude as a constraint on the norm induced by $\Sigma$.
% Formally, we use the constraint $\|\pmb{\delta}\|_{\Sigma, 2} \leq 1$
% \footnote{Note that this formulation still allows for bounding $\|\pmb{\delta}\|_{\Sigma, 2}$ by an $\epsilon > 0$, rather than by $1$, as is more common in adversarial robustness. This is trivially achieved by defining $\Sigma$ slightly different, as $\Sigma \coloneqq \nicefrac{1}{\epsilon^2}\:\Sigma$.}, 
% where $\|\pmb{\delta}\|_{\Sigma, 2} = \sqrt{M_\Sigma(\pmb{\delta},\pmb{\delta})} = \sqrt{\pmb{\delta}^\top\Sigma\:\pmb{\delta}}$, and so the allowable magnitude of the perturbation is controlled solely by $\Sigma$.

% \textit{\textbf{Summary.}} Given the previous definitions for the direction and magnitude constraints, we propose to define the set of semantically-viable perturbations as $\mathcal{S}(V, \Sigma) = \{V^\top\pmb{\delta} \: : \: \|\pmb{\delta}\|_{\Sigma, 2} \leq 1\}$.
% Analogously, we define semantically-viable variants of image $I$, produced by latent code $\mathbf{z}$, \ie $I = G(\mathbf{z})$, as the set of images $\mathcal{V}(I) = \{G(\mathbf{z} + \pmb{\eta}) \: : \pmb{\eta} \in \mathcal{S}(V, \Sigma)\}$. 

% For a fixed $G$ and $I$. the sensibleness of the actual semantic viability of images in $\mathcal{V}(I)$ is controlled by a sensible choosing of $V$ and $\Sigma$.
% In Section~\ref{sec:pract_cons} we introduce a methodology for choosing these two elements such that the images in $\mathcal{V}(I)$ hold up to a reasonable level of human scrutiny.


% \subsection{Semantically-viable Adversarial Attacks}
% Given our formalization of the set of semantically-viable perturbations, we adapt standard adversarial attacks to our methodology.
% We consider two types of attacks, which differ in how the perturbation's norm is used.
% This norm is used either as a constraint (\ie constrained-perturbation attacks) or as the objective (\ie minimum-perturbation attacks).
% Next, we show how we adapt each type of attack.

% \subsubsection{Constrained-perturbation attacks}
% The constrained-perturbation rationale casts an attacking as a maximization of a loss function over a constrained set of inputs such that the target model is fooled.
% A widely-used procedure for achieving this is Projected Gradient Descent (PGD), which we explain next.

% \textbf{Standard PGD Attacks.} 
% These attacks are usually a variant of gradient ascent over the loss function, with the additional step of projecting the optimization's current iterate to the set of viable inputs.
% Formally, the task is attacking a classification model $f$, that maps from the space of images to the probability simplex over the set of classes $\mathcal{Y}$, \ie $f: \mathcal{I} \to \mathcal{P}(\mathcal{Y})$.
% In particular, when searching for an adversarial perturbation for model $f$ at input image $\mathbf{x}$ with corresponding label $y$, PGD attacks perform iterations of
% \begin{equation}\label{eq:usual_step}
%     \pmb{\eta}^{t+1} = \prod_{\mathcal{B}} g\left(\pmb{\eta}^t, \nabla_{\pmb{\eta}^t}\mathcal{L}(f(\mathbf{x} + \pmb{\eta}^t), y)\right),
% \end{equation}
% where $\prod_{\mathcal{B}}\mathbf{x}$ denotes the projection of $\mathbf{x}$ onto set $\mathcal{B}$ (the set of allowable perturbations--usually an $\ell_p$ ball of fixed radius), $g$ is the optimizer, and $\mathcal{L}$ is the loss function to be maximized.

% \textbf{Adaptation to our methodology.} To combine standard PGD attacks, \ie Equation~\ref{eq:usual_step}, with our methodology, we perform the following modifications.
% First, instead of image-label pairs, we consider latent code-label pairs, \ie $\mathbf{z}$ with corresponding label $y$.
% Second, since we search for $\pmb{\eta}$ in the latent space instead of the image space, we perturb $\mathbf{z}$ instead of $\mathbf{x}$.
% Third, we exploit the generator $G$'s differentiability, and introduce $G$ into the expression so that the latent codes can be mapped to image space.
% Finally, we set $\mathcal{B}$ to be $\mathcal{S}(V, \Sigma)$.
% These modification imply that our adaptation of the usual PGD attacks performs repeated iterations of
% \[
% \pmb{\eta}^{t+1} = \prod_{\mathcal{S}(V, \Sigma)} g\left(\pmb{\eta}^t, \nabla_{\pmb{\eta}^t}\mathcal{L}(f(G(\mathbf{z} + \pmb{\eta}^t)), y)\right).
% \]

% However, we note that searching for $\pmb{\eta} \in \mathcal{S}(V, \Sigma)$ is equivalent to searching for $\pmb{\delta}$ such that $\|\pmb{\delta}\|_{\Sigma, 2} \leq 1$ and then computing $\pmb{\eta} = V^\top\pmb{\delta}$. 
% This simplification implies reducing the search space from $\mathbb{R}^d$ to $\mathbb{R}^N$ (\ie searching for $\pmb{\eta}$ \textit{vs.} searching for $\pmb{\delta}$).
% When $N \ll d$, as is most likely for semantic directions, this simplification can have significant impact in computational cost.
% Thus, the final form of our search is
% \begin{equation}\label{eq:our_step}
%     \pmb{\delta}^{t+1} = \prod_{\pmb{\delta} : \|\pmb{\delta}\|_{\Sigma, 2} \leq 1} g\left(\pmb{\delta}^t, \nabla_{\pmb{\delta}^t}\mathcal{L}(f(G(\mathbf{z} + V^\top\pmb{\delta}^t)), y)\right).
% \end{equation}

% Equation~\eqref{eq:our_step} shares several features with Equation~\eqref{eq:usual_step}, except for the projection step.
% In particular, while Equation~\eqref{eq:usual_step} requires projecting points to $\ell_p$ balls, Equation~\eqref{eq:our_step} requires projecting points to the region defined by $\|\pmb{\delta}\|_{\Sigma, 2} \leq 1$.
% This region, since $\Sigma$ is symmetric and PD, is an ellipsoid; thus, our projection step implies projecting points to the ellipsoid defined by $\Sigma$.
% Here we note that projecting to ellipsoids is not as straightforward as projecting to $\ell_p$ balls.
% Thus, we next derive an inexpensive procedure for projecting to ellipsoids.
% Our procedure allows the projection step to have a low cost, allowing, in turn, the iterative attack itself to be computationally tractable.

% \textbf{Projecting to ellipsoid.} Formally, projecting a point $\pmb{\delta}$ to the region defined by $\|\pmb{\delta}\|_{\Sigma, 2} \leq 1$ is defined as solving
% \begin{equation}\label{eq:project}
%     \arg\min_{\pmb{\delta}_*} \frac12\:\|\pmb{\delta}_* - \pmb{\delta}\|_2^2,\qquad\text{s.t. } \pmb{\delta}_*^\top\Sigma\:\pmb{\delta}_*\leq1.
% \end{equation}
% If $\pmb{\delta}$ is already inside the ellipse, then $\pmb{\delta}_* = \pmb{\delta}$.
% Otherwise, we are tasked with solving Problem~\eqref{eq:project} but replacing the inequality constraint with an equality, \ie searching for $\pmb{\delta}_*$ on the surface of the ellipse.
% To solve this optimization problem the Lagrangian is
% \[
%     L(\delta^*, \lambda) = \frac12\:\|\pmb{\delta}_* - \pmb{\delta}\|_2^2 + \lambda\:\left(\pmb{\delta}_*^\top\Sigma\:\pmb{\delta}_* - 1\right).
% \]
% % Deriving the KKT conditions of this problem yields:
% Differentiating w.r.t. $\pmb{\delta}_*$, using the fact that $\Sigma$ is symmetric, and equating to zero yields 
% \begin{equation}\label{eq:delta_star}
%     \left(I + \lambda\:\Sigma\right)\pmb{\delta}_* = \pmb{\delta}.
% \end{equation}
% On the other hand, differentiating w.r.t. $\lambda$ and equating to zero yields 
% \begin{equation}\label{eq:constraint}
%     \pmb{\delta}_*^\top\Sigma\:\pmb{\delta}_* - 1 = 0.
% \end{equation}
% By combining Equations~\eqref{eq:delta_star} and~\eqref{eq:constraint} we arrive at
% \begin{equation}\label{eq:find_root}
%     \pmb{\delta}^\top \left(I + \lambda\:\Sigma\right)^{-1}\Sigma\left(I + \lambda\:\Sigma\right)^{-1}\pmb{\delta} - 1 = 0.
% \end{equation}
% The only unknown in Equation~\eqref{eq:find_root} is $\lambda$.
% If we let the LHS of Equation~\ref{eq:find_root} be $h(\lambda)$, then we can see that solving for $\lambda$ is equivalent to finding $\lambda_*$, the root of $h$.
% Once $\lambda_*$ is found, we can directly find $\pmb{\delta}_*$ by substituting $\lambda_*$ into Equation~\ref{eq:delta_star} and solving the linear system for $\pmb{\delta}_*$, which is an efficient operation.
% Thus, our task of finding the vector $\pmb{\delta}_* \in \mathbb{R}^N$ is reduced to finding the scalar $\lambda_*$ and solving a linear system.

% Since $\lambda_*$ is a scalar, finding the root of $h$ can be done efficiently through traditional numerical optimization methods.
% In this work, we use the bisection method to find $\lambda_*$.

% \subsubsection{Minimum-perturbation Attacks}
% The minimum-perturbation rationale casts an attack as the minimization of a perturbation's norm such that the target model is fooled.
% While constrained-perturbation attacks aim at finding a perturbation whose norm is smaller than a fixed value, minimum-perturbation attacks aim at finding the smallest perturbation that fools the model.
% Here we report how we adapt FAB, a state-of-the-art minimum-perturbation attack, to our methodology.

% \textbf{Main algorithmic modifications.}
% FAB's algorithm aims at minimizing the $\ell_p$ norm of a perturbation $\pmb{\delta}$.
% There are versions of FAB for each $p \in \{1,2,\infty\}$.
% We extend FAB to our methodology by modifying the algorithm to consider the norm induced by our $\Sigma$ matrix, \ie $\|\pmb{\delta}\|_{\Sigma, 2}$.

% Such modification amounts to adjusting the $p = 2$ version of the attack for our purposes.
% Specifically, we (1) replace inner products in the $p$ norm, \ie $\mathbf{u}^\top\mathbf{v}$, by $\mathbf{u}^\top\Sigma\mathbf{v}$, (2) replace inner products in the dual norm $q$ by $\mathbf{u}^\top\Sigma^{-1}\mathbf{v}$ (where $\nicefrac{1}{p} + \nicefrac{1}{q} = 1$), and (3) re-implement the projection operations required inside FAB's algorithm.
% Further, for initializing the adversarial perturbation, we perform random initialization by uniform sampling inside the ellipsoid parameterized by $\Sigma$, through the procedure we report in Section~\ref{sec:pgd_adv}.


% \subsubsection{Interpreting the Adversarial Perturbations}
% The adversarial perturbations $\pmb{\delta}$ enjoy the property of being inherently interpretable.
% Here describe the definition of the budget spent on each attribute: how to obtain a candidate ranking and then statistically evaluate the ranking through paired statistical tests.
% Friedman's test, weighed votes and the Wilcoxon signed-rank test.


% \subsection{Certification Against Semantic Perturbations}
% % \textcolor{red}{We might need to have the face recognition part before the certification.}
% Our methodology considers a model $f$ that classifies the output of a generative model $G$ when the latter is provided with a particular latent code $\mathbf{z}$.
% For ease of notation, we consider the composition $F(\mathbf{z}) = f(G(\mathbf{z})) : \mathbb{R}^d \rightarrow \mathcal P(\mathcal{Y})$.
% % Thus, classifier $f(x)$ maps the generated input image to the probability simplex $\mathcal P(Y)$ over the set of classes $\mathcal Y$. 
% With this notation, we specialize the definition of domain-smoothed classifiers~\cite{deformrs} to smooth semantic perturbations defined by matrix $V$.

% \begin{definition}\label{def:smooth-classifier}
% Given a classifier $F(\mathbf{z}): \mathbb{R}^d \rightarrow \mathcal P(Y)$, we define a semantically-smoothed classifier as:
% \[    
% g(\mathbf{z}, \mathbf{p}) = \mathbb{E}_{\pmb{\epsilon}\sim \mathcal N(0, \Sigma)}\left[F\left(\mathbf{z} + V^T(\mathbf{p}+\pmb{\epsilon})\right) \right].
% \]
% \end{definition}

% In a nutshell, $g$'s prediction for the image generated from latent code $\mathbf{z}$ is the expected value of $F$'s predictions of semantically-perturbed variants of such image, where these variants are obtained by perturbing $\mathbf{z}$. 
% With the following proposition we show that our smooth classifier $g$ is certifiably robust against semantic perturbations.
% We leave the proof for the \textbf{Supplementary Materials}.

% \begin{proposition}\label{prop:semantic-perturbation-certification}
% Let $g$ assigns the class $c_A$ for the input pair $(z, p)$, \ie $\text{arg}\max_c g^c(z, p) = c_A$ with:
% \[
% p_A = g^{c_A}(z, p) \quad\text{and}\quad p_B = \max_{c \neq c_A} g^c(z, p)
% \]
% then $\text{arg}\max_c g^c(z, p+\delta) = c_A \,\, \forall \delta$ satisfying
% \begin{equation}\label{eq:certification}
%     \sqrt{\delta^T \Sigma^{-1} \delta} \leq \frac{1}{2}\left(\Phi^{-1}(p_A) - \Phi^{-1}(p_B) \right).
% \end{equation}
% \end{proposition}
% Proposition \ref{prop:semantic-perturbation-certification} states that: as long as the the semantic perturbation $\delta$ is within the ellipsoidal region defined by equation \eqref{eq:certification}, then the smooth classifier $g$ will not alter its prediction from $c_A$. It is worthwhile mentioning that, while we chose our semantic perturbations $V$ to be associated with a GAN latent space, this result is generic to any semantic direction $V$. That is to say, for any set of characterized semantic perturbations through a matrix $V$, our smooth classifier $g$ is certifiable against such semantic perturbations. 

\section{Practical considerations}\label{sec:pract_cons}
We have presented our methodology for exploring semantically-viable adversarial examples.
Our methodology is based on our definition of the space of semantically-viable perturbations.
In this section, we present practical considerations for implementing our methodology.
In particular, we put forward the difficulties we found when trying to define: (1) the space of semantically-viable perturbations, (2) the details of the PGD-based adversary to be used, and (3) the image domain in which to test our methodology.

\subsection{The Space of Semantically-viable Perturbations}\label{sec:space}
We propose a methodology for exploring semantically-viable perturbations of images.
We argue that no methodology aiming at exploring semantically-viable perturbations of images can ensure that the perturbations will indeed be semantically viable.
That is, we argue that all methodologies aiming at this task, ours not being the exception, will produce images that will deviate from the assumption of ``semantically viable'' (at least to some extent).
The reason behind this fundamental difficulty is that modeling semantics in images is still one of the core challenges in computer vision.

Despite this hindrance, our methodology provides a set of ``knobs'' that allow tuning how much the examples we find deviate from the assumption of semantic viability.
In particular, assuming a sufficiently powerful image-generation process (modeled by generator $G$ in our methodology), we argue that this deviation can be controlled by a sensible choosing of $V$ and $\Sigma$.
Next, we present our methodology for selecting these two items.

\textbf{Defining $V$.}
Matrix $V$ is the set of directions associated with semantic attributes in an image.
For choosing $V$, we exploit the fact our methodology models the image-generation process with a GAN.
We draw upon recent advances in research on the interpretation of the representations learnt by GANs.
This area of research aims at studying the latent space learnt by GANs in the pursuit of discovering interpretable directions.
Such discovered directions are interpretable in the sense that perturbing samples along them allows control, to a reasonable extent, of semantically-meaningful visual characteristics.
% These characteristics can be domain-independent, \eg viewpoint, lighting, time of day, or strongly domain-dependent, \eg smile, pose, aging in the case of human faces.

Given a trained GAN, recent methods for the task of latent space interpretation find a set of directions in the GAN's latent space, represented by vectors.
These methods also establish, for each direction, a particular semantic attribute with which the corresponding direction is associated.
In this work, we choose the set of directions associated with semantic attributes in the image, as introduced in Section~\ref{sec:semantic_perturbs}, to be the directions found by a GAN interpretation method.
That is, we assume reasonable performance of these methods, and so build matrix $V$ by vertically stacking the set of directions $\{\mathbf{v}_i\}_{i=1}^n$ produced by one such method.
We underscore, however, that this design choice is independent of our methodology.
Specifically, while this choice allows us to empirically validate our approach, better choices may exist, yielding better empirical results.
Thus, our approach can benefit from advances in the area of interpretability of generative models.

\textbf{Defining $\Sigma$.}
Matrix $\Sigma$ characterizes the ellipsoidal region of valid perturbations $\pmb{\delta}$ by controlling the perturbation's norm via $\|\pmb{\delta}\|_{\Sigma, 2} \leq 1$.
Each entry of $\pmb{\delta} \in \mathbb{R}^N$ is associated with one of the $N$ directions $\{\mathbf{v}_i\}_{i=1}^N$, which, in turn, corresponds to a semantic attribute.
Defining $\Sigma$'s entries, thus, can be associated with the amount of perturbation we allow for each of $\pmb{\delta}$'s entries. 
Our definition of $\Sigma$ is thus based on the \textit{maximum} amount of perturbation allowed along each individual direction $\mathbf{v}_i$.
In particular, let the scalar $\epsilon_i$ state the maximum extent to which latent codes can be perturbed in the direction of $\mathbf{v}_i$.
This $\epsilon_i$ is ``maximal'' in the sense that semantically-invalid modifications would be introduced if the perturbation was larger than $\epsilon_i$.
Thus, we require $\Sigma$ to account for the fact that the magnitude of each entry of $\pmb{\delta}$ must not exceed its corresponding $\epsilon$ or, formally, $|\pmb{\delta}_i| \leq \epsilon_i$.

Furthermore, since $\Sigma$ must, by construction, define an ellipsoidal region, we relate the above requirement with a geometrical reasoning.
Specifically, we note that our requirements for $\Sigma$ imply that the associated ellipse must pass through the $N$ points $\mathbf{p}_1 = [\epsilon_1, 0,\:\dots,\:0]^\top$, $\mathbf{p}_2 = [0, \:\epsilon_2, \:\dots,\:0]^\top$, \dots, $\mathbf{p}_N = [0, \:\dots,\:\epsilon_N]^\top$.
To account for the absolute value in our requirement, the ellipse must also pass through $-\mathbf{p}_1$, $-\mathbf{p}_2$, \dots, $-\mathbf{p}_N$.
Thus, this $N$-dimensional ellipse must pass through the set of $2N$ points $\mathcal{P} = \{\mathbf{p}_i\}_{i=1}^N \cup \{-\mathbf{p}_i\}_{i=1}^N$, which are a function of $\{\epsilon_i\}_{i=1}^N$.

However, this constraint is insufficient to uniquely define the ellipse: there is an infinite set of ellipses that comply with the constraint.
We note that our requirement of $|\pmb{\delta}_i| \leq \epsilon_i$ also implies that the ellipse must not simply pass through the points in $\mathcal{P}$, but also that these points should be the ellipse's extrema.
Hence, $\Sigma$ is defined as a matrix parameterizing the ellipse whose extrema are the points in $\mathcal{P}$.
Equivalently, we are searching for the $\Sigma$ that parameterizes an ellipse that passes through these points and encloses the minimum volume, which is equivalent to the $\Sigma$ whose determinant is maximal~\cite{boyd2004convex}.

Given a set of points, such $\Sigma$ can be found with the algorithm introduced in~\cite{moshtagh2005minimum}.
However, we note that the points in $\mathcal{P}$ enjoy properties that can simplify the search for $\Sigma$.
In particular, the set of points $\mathcal{P}$ is composed of scaled versions of the canonical basis for $\mathbb{R}^N$.
This fact implies that the ellipse we are searching for has its semi-axis aligned with the canonical axis of $\mathbb{R}^N$.
Thus, we can simply define $\Sigma$ as a diagonal matrix whose elements are the reciprocal of the squares of the $\epsilon$, that is 
\begin{equation}\label{eq:sigma_def}
    \Sigma = \begin{bmatrix}
    \epsilon_1^{-2} &                   & \\
                    & \ddots            & \\
    &               & \epsilon_N^{-2}
  \end{bmatrix} = \text{diag}(\epsilon_1^{-2},\:\dots, \:\epsilon_N^{-2}).
\end{equation}

\subsubsection{Impact of $\Sigma$ on computation}
Here underscore how we can exploit our definition of matrix $\Sigma$ to reduce computation in our methodology.
Note that $\Sigma$ is used in the procedure for projecting perturbations to the ellipsoid.
In particular, projections are performed by first solving for $\lambda$ in Equation~\eqref{eq:find_root} and then using such solution to solve for $\pmb{\delta}_*$ in Equation~\eqref{eq:delta_star}.
Equation~\eqref{eq:find_root} involves $\Sigma$ for one inversion and for two matrix multiplications.
However, since we defined $\Sigma$ to be a diagonal matrix (as in Equation~\ref{eq:sigma_def}), we can simplify Equation~\eqref{eq:find_root} to
\[
    \sum_{i=1}^N \frac{\pmb{\delta}_i^2\epsilon_i^{-2}}{\left(1 + \lambda\epsilon_i^{-2}\right)^2} - 1 = 0,
\]
which does not require matrix multiplication nor inversion.
Moreover, the system in Equation~\eqref{eq:delta_star} can be efficiently solved via inversion since the associated matrix is diagonal.
Thus, in our implementation, we exploit these observations to lower the computational expense of projecting the perturbations at each iteration of PGD.

Similarly, the diagonal property of $\Sigma$ is exploited across our implementation when $\Sigma$ is the matrix involved in a bilinear form.
Such implementation trick reduces the computational complexity of these matrix multiplications.

\textit{\textbf{Summary.}}
We define $V$ by constructing upon recent work in the domain of interpreting the latent space of GANs.
In particular, $V$ is defined in terms of the semantic directions that are found by methods from the GAN-interpretation domain.
Further, we define $\Sigma$ as a diagonal matrix whose entries are a function of the tunable hyper-parameters related to the maximal amount of perturbation allowed along each semantic direction \ie the $\epsilon_i$'s.
Specifically, we define $\Sigma$ such that it parameterizes a minimal-volume ellipsoid that passes through a set of points defined by the $\epsilon_i$'s.
Defining both $V$ and $\Sigma$ completes our definition of the space of semantically-viable perturbations.


% \subsubsection{PGD Adversary}\label{sec:pgd_adv}
% Most works on adversarial robustness use Projected Gradient Descent (PGD) to find perturbations.
% Furthermore, most of these works study perturbations in the pixel space.
% In contrast, our methodology studies perturbation in latent space.
% Thus, some modifications to the PGD-based adversary are required.
% Here we report a set of practical considerations this PGD-based adversary must follow to work under our methodology.

% \textbf{Adversary Initialization.}
% Previous works on adversarial robustness have shown that the initialization of the adversarial perturbation $\pmb{\delta}$ can have sizable impact in the performance of the attack~\cite{Wong2020Fast}.
% Interestingly, Wong \textit{et al.}~\cite{Wong2020Fast} found that initializing the perturbation to random noise within the space of perturbations dramatically increases performance.
% By analogy, together with our methodology, we report the procedure for randomly initializing the perturbation, with the modifications induced by our formalization of the space of perturbations.

% In particular, we recall that our methodology models the space of perturbations as the volume enclosed by the ellipsoid parameterized by the matrix $\Sigma$.
% Thus, we are interested in randomly initializing $\pmb{\delta}$ uniformly within such volume.
% To achieve this, we first initialize $\pmb{\delta}$ uniformly within the unit ball and then deform the ball to the ellipsoid parameterized by $\Sigma$ by performing Cholesky decomposition.
% We report details on this procedure in the \textbf{Supplementary Material}.

% \textbf{Optimizer.}
% Empirically, we found that off-the-shelf usage of Gradient Descent does not perform well for finding adversaries.
% Specifically, naively using the SGD optimizer is not sufficient for finding adversaries.
% By exploring more sophisticated optimizers, we found that the Adam optimizer~\cite{kingma2014adam} works remarkably better than SGD.
% Further, extensive experimentation yielded results showing that Adam must be coupled with a relatively large learning rate of $1.0$ to successfully find adversaries.


% \subsubsection{The Domain of Images}
% Our methodology's strongest assumptions are (1) that GANs can generate images that align with real-world data, and (2) that the methods for interpreting the latent space of GANs can find directions that correlate with so-called ``semantic attributes''.
% Deviations from these assumptions thus have an impact in the results achieved by employing our methodology.
% While both GANs and GAN-interpretation methods have flourished in recent years, our assumptions hold the strongest for \textit{restricted} domains of images.
% Thus, for showcasing our methodology, we choose a specific domain of images in which both GANs and GAN-interpretation methods excel: human faces.

% Note that choosing this domain implies that the systems we will target for attacks are Face Recognition Models (FRMs).
% The selection of both this domain and these recognition systems brings a set of benefits, which we outline next.
% First, while the definition of ``semantic attribute'' can be loose and contended in the domain of general images, the consensus on the definition increases for images of human faces; in practice, such consensus allows us to broadly speak in terms of attributes such as ``smiling'' or ``pose''.
% Second, FRS are frequently deployed in the real world for security-critical purposes; thus, developing understanding of their failure modes against semantic perturbations is of value for both the research community and industry.
% Third, FRS are domain-specific systems, allowing them to enjoy particularly high performances on current datasets; hence, we argue that identifying flaws in their performance with our methodology will be informative of real-world phenomena, rather than just discovering artifacts that could arise when targeting lower-performing systems.




% In the next section, we leverage our methodology to assess and characterize the semantic robustness of Face Recognition Models.



==> Tables/attr_ranking_fab.tex <==
\begin{table*}[]
\centering
\caption{\textbf{Ranking of budget spent by FAB on each attribute.} 
Rankings for FAB's expenses on each attribute (generated with the methodology described in Section~\ref{sec:interpreting}). 
This ranking suggests the relative extent to which FRM's rely on a particular attribute. 
We denote the statistically-significant pair-wise comparisons with ``$>^\star$'', and the rest with ``$\geq$'' (all comparisons with a significance of $\alpha = 0.01$). 
We report the number of samples for each pair-wise statistical test in the last column, while we report the corresponding \textit{p}-values in the \textbf{Supplementary Materials}.
\label{tab:deltas_fab}}
\vspace{-0.3cm}
\begin{tabular}{c|C{1.4cm}cC{1.4cm}cC{1.4cm}cC{1.4cm}cC{1.4cm}|c}
\hline
\multirow{2}{*}{Method} & \multicolumn{9}{c|}{Ranking} &  \multirow{2}{*}{$n$}  \\
        & 1$^{\text{st}}$        &                & 2$^{\text{nd}}$        &                & 3$^{\text{rd}}$        &                & 4$^{\text{th}}$        &                & 5$^{\text{th}}$        & \\ \hline\hline
ArcFace & Gender & $>^\star$ & Pose & $>^\star$ & Eyeglasses & $>^\star$ & Age & $>^\star$ & Smile & 5000 \\
FaceNet$^C$ & Gender & $>^\star$ & Eyeglasses & $\geq$ & Pose & $>^\star$ & Age & $>^\star$ & Smile & 5000 \\
FaceNet$^V$ & Eyeglasses & $\geq$ & Pose & $>^\star$ & Gender & $>^\star$ & Age & $>^\star$ & Smile & 5000 \\\hline
\end{tabular}
\end{table*}

==> Tables/pgd_budget.tex <==
\begin{table}[]
\centering
\caption{\textbf{Varying the perturbation's constraint in PGD attacks.} 
We vary the amount of allowable perturbation, and record the robustness of each method when conducting PGD attacks with such perturbation.
\label{tab:pgd_dataset}}
\centering
\begin{tabular}{c|cccccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{6}{c}{Robustness over perturbation budget} \\
                        & $\nicefrac{1}{8}\:\Sigma$ & $\nicefrac{1}{4}\:\Sigma$ & $\nicefrac{1}{2}\:\Sigma$ & $1\:\Sigma$   & $2\:\Sigma$   & $4\:\Sigma$              \\ \hline\hline
ArcFace                 & 4.1                       & 24.9                      & 60.4                      & 84.9          & 95.2          & 98.3 \\
FaceNet$^\text{C}$      & 12.6                      & 33.6                      & 58.3                      & 76.9          & 89.0          & 95.4   \\
FaceNet$^\text{V}$      & 7.3                       & 25.1                      & 50.4                      & 71.0          & 85.2          & 93.3  \\\hline
\end{tabular}
\end{table}

==> Tables/pgd_on_nids.tex <==
\begin{table}[]
\centering
\caption{\textbf{Varying the number of attacked instances in PGD attacks.} 
We vary the amount of attacked instances, and record the robustness of each method when conducting PGD attacks.
\label{tab:pgd_attackedinstances}}
\centering
\begin{tabular}{c|ccccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c}{Robustness with attacks on $n$ identities} \\
                        & \verb'1k'     & \verb'2.5k'   & \verb'5k'     & \verb'10k'    & \verb'20k'\\ \hline\hline
ArcFace                 & 85.3          & 84.8          & 84.9          &  85.2         & 85.4   \\
FaceNet$^\text{C}$      & 77.1          & 77.0          & 76.9          &  77.5         & 77.6    \\
FaceNet$^\text{V}$      & 72.2          &  71.0         & 71.0          & 71.7          & 71.9     \\\hline
\end{tabular}
\end{table}

==> Tables/pgd_over_nids.tex <==
\begin{table}[]
\centering
\caption{\textbf{Varying the database's size in PGD attacks.} 
We vary the amount of instances in the database, and record the robustness of each method when conducting PGD attacks.
\label{tab:pgd_sigma}}
\centering
\begin{tabular}{c|cccccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{6}{c}{Robustness over $n$-identity dataset} \\
                        & \verb'5k'     & \verb'10k'    & \verb'50k'    & \verb'100k'   & \verb'500k'   & \verb'1M' \\ \hline\hline
ArcFace                 & 93.0          & 91.4          & 86.8          & 84.9          & 79.8          & 77.9  \\
FaceNet$^\text{C}$      & 85.5          & 83.5          & 78.6          & 76.9          & 72.7          & 70.9  \\
FaceNet$^\text{V}$      & 81.4          & 79.0          & 73.1          & 71.0          & 66.8          & 64.7  \\\hline
\end{tabular}
\end{table}
